Tracking the Best Beam for a Mobile User via Bayesian Optimization

The standard beam management procedure in 5G requires the user equipment (UE) to periodically measure the received signal reference power (RSRP) on each of a set of beams proposed by the basestation (BS). It is prohibitively expensive to measure the RSRP on all beams and so the BS should propose a beamset that is large enough to allow a high-RSRP beam to be identified, but small enough to prevent excessive reporting overhead. Moreover, the beamset should evolve over time according to UE mobility. We address this fundamental performance/overhead trade-off via a Bayesian optimization technique that requires no or little training on historical data and is rooted on a low complexity algorithm for the beamset choice with theoretical guarantees. We show the benefits of our approach on 3GPP compliant simulation scenarios.

==> BOrefinements.tex <==
\section{Algorithm Refinements}
\label{sec:BOrefinements}

\textcolor{red}{To be discarded in case of lack of space}

\noindent \textbf{Learning the kernel from historical data.} \textcolor{red}{This could be useful to justify the case with exotic beam dictionaries.}
When the choice of the kernel and/or of kernel distance $\delta$ is not straightforward but historical observations $\mathcal D$ are available, one can resort to a \emph{meta-learning} technique \cite{rothfuss2021pacoh}. The metric $\delta$ computing the distance between points in $\mathcal X$ is defined as
\begin{equation} \label{eq:delta_iheta}
	\delta_\theta(x,x') := \|h_\theta(x) - h_\theta(x')\|_2^2
\end{equation}
where $h_{\theta}$ is a neural network with weights $\theta$ and the kernel $k$ can be simply re-defined as
\begin{equation} \label{eq:param_kernel}
	k_{\theta}(x,x') := \exp\left( -\delta_\theta(x,x') \right), \quad \forall\, x,x'\in \mathcal X
\end{equation}
Then, $\theta$ is optimized by maximizing the log-likelihood of historical observations:
\begin{equation} \label{eq:theta_opt}
	\bar{\theta} = \argmax_{\theta} \log p \left( \mathbf{f} | \mathbf{x} \right), \qquad \mathrm{where} \ \mathcal D=\{\mathbf x, \mathbf f\}
\end{equation}
Intuitively, $h_{\bar{\theta}}$ captures those $(x,x')$ pairs whose reward are highly correlated (i.e., for which $h_{\bar{\theta}}(x)\approx h_{\bar{\theta}}(x)$ thus $k_{\bar{\theta}}(x,x')\approx 1$) to efficiently infer $f(x')$ when observing $f(x)$. 

Similarly, as new observations are collected in online fashion and added to $\mathcal D$, NN weights are re-optimized as in \eqref{eq:theta_opt}.





==> related_works.tex <==









